Antisymmetric Wilson loops in N = 4 SYM: from exact results to non-planar corrections

We consider the vacuum expectation values of 1/2-BPS circular Wilson loops in N=4 super Yang-Mills theory in the totally antisymmetric representation of the gauge group U(N) or SU(N). Localization and matrix model techniques provide exact, but rather formal, expressions for these expectation values. In this paper we show how to extract the leading and sub-leading behavior in a 1/N expansion with fixed 't Hooft coupling starting from these exact results. This is done by exploiting the relation between the generating function of antisymmetric Wilson loops and a finite-dimensional quantum system known as the truncated harmonic oscillator. Sum and integral representations for the 1/N terms are provided.

==> GF.tex <==
\subsection{Generating Function}
\label{GF}
The precise relation between the circular Wilson loop and the Gaussian matrix model is
\begin{empheq}{equation}\label{GF:WL.UN}
	\vev{W_R}_{U(N)} =\frac{1}{\textrm{dim}[R]}\vev{\Tr_R \left[\e{X}\right]}\,,
\end{empheq}
where $R$ denotes the representation of the $U(N)$ gauge group and $\Tr_R$ the corresponding trace. The vacuum expectation value on the left is defined on the $\mathcal{N}=4$ SYM theory; the right hand side corresponds to an insertion in the matrix model. 

In this paper we will be concerned with the totally antisymmetric representation of rank $k$ defined by the Young diagram
\begin{empheq}{equation}
	\mathcal{A}_k =\left.\substack{\yng(1,1)\vspace{-0.15cm}\\\vdots\vspace{0.05cm}\\\yng(1)}\right\}k\,.
	\qquad
	k\leq N\,.
\end{empheq}
It has dimension 
\begin{empheq}{equation}
	\textrm{dim}[\mathcal{A}_k]=\binom{N}{k}\,.
\end{empheq}
The structure of the trace $\Tr_{\mathcal{A}_k}$ can get increasingly complicated as the rank $k$ grows. Indeed, for any $N\times N$ matrix $X$ we have
\begin{empheq}{align}
	\Tr_{\mathcal{A}_1} X &=\Tr X\,,
	\\
	\Tr_{\mathcal{A}_2} X &=\frac{1}{2}\left(\Tr X \right)^2-\frac{1}{2}\Tr\left(X^2\right)\,,
	\\
	\Tr_{\mathcal{A}_3} X &=\frac{1}{6}\left(\Tr X\right)^3 -\frac{1}{2}\Tr\left(X^2\right)\Tr X +\frac{1}{3}\textrm{Tr}\left(X^3\right)\,,
\end{empheq}
and so forth. Happily, there is a natural way to encode this structure into the generating function
\begin{empheq}{equation}\label{GF:FA.def}
	F_A(t;X)\equiv\det\left[1+tX\right]=\sum_{k=0}^N t^k \Tr_{\mathcal{A}_k}[X] \,.
\end{empheq}

A straightforward calculation using \eqref{MM:I.def}, \eqref{MM:Deltat.def} and \eqref{MM:vev.def} reveals that the matrix model expectation value of this generating function is 
\begin{empheq}{equation}\label{GF:F.exact}
	\vev{F_A(t;\e{X})}_{U(N)}=\det \left[I(y,z)+t\e{\frac{g^2}{2}}I(g+y,g+z)\right]=\det \left[1+t\e{\frac{g^2}{2}}I(g,g)\right]\,.
\end{empheq}
The dependence on $y$ and $z$ disappears as a consequence of \eqref{MM:I.propexp} and $\det I(g,g)=1$.

Before going on, let us mention how to reproduce the result of Fiol and Torrents \cite{Fiol:2013hna} from \eqref{GF:F.exact}. Consider the matrix $I(g,g)$ given explicitly in \eqref{MM:I.expl}. If one multiplies the $m$-th row of this matrix by $\sqrt{(m-1)!}\, g^{-m}$ and divides the $m$-th column by the same factor, the determinant in \eqref{GF:F.exact} does not change. Hence, one finds 
\begin{empheq}{equation}
	\vev{F_A(t;\e{X})}_{U(N)} = \det\left[ 1 + t \e{\frac12 g^2} \tilde{I}(g,g) \right]~, \qquad 
	\tilde{I}_{mn}(g,g)= \Laguerre^{(m-n)}_{n-1}(-g^2)\,,
\end{empheq}
which is the expression given by Fiol and Torrents. Note that our generating functional differs by a factor of $t^N$ from theirs.


In the answer \eqref{GF:F.exact} we recognize the form of the generating function of antisymmetric traces \eqref{GF:FA.def} for the matrix $I(g,g)$, 
\begin{empheq}{equation}\label{GF:W.trace}
	\vev{F_A(t;\e{X})}=F_A\left(t\e{\frac{\lambda}{8N}};I(g,g)\right)~,
\end{empheq}
which allows us, using \eqref{GF:FA.def} and \eqref{GF:WL.UN}, to obtain the formal yet remarkably simple result
\begin{empheq}{equation}\label{GF:WL.UN.simple}
	\vev{W_{\mathcal{A}_k}}_{U(N)}=\frac{1}{\textrm{dim}[\mathcal{A}_k]} \e{\frac{\lambda k}{8N}}\Tr_{\mathcal{A}_k} [I(g,g)]\,.
\end{empheq}
For the gauge group $SU(N)$, the matrix model must be restricted to traceless matrices. This can be achieved either by using a Lagrange multiplier or by explicitly isolating the trace component in the matrix model integral, as was done in \cite{Gordon:2017dvy}. The outcome is
\begin{empheq}{equation}\label{GF:WL.SUN.simple}
	\vev{W_{\mathcal{A}_k}}_{SU(N)}=\vev{W_{\mathcal{A}_k}}_{U(N)}\e{-\frac{\lambda k^2}{8N^2}}
	=\frac{1}{\textrm{dim}[\mathcal{A}_k]}\e{\frac{\lambda k(N-k)}{8N^2}}\Tr_{\mathcal{A}_k}[I(g,g)]\,.
\end{empheq}
Because the representations $\mathcal{A}_k$ and $\mathcal{A}_{N-k}$ are conjugate to each other for the gauge group $SU(N)$, we expect $\vev{W_{\mathcal{A}_k}}_{SU(N)}=\vev{W_{\mathcal{A}_{N-k}}}_{SU(N)}$. This can be demonstrated by noting that, for an invertible matrix $X$, \eqref{GF:FA.def} implies 
\begin{empheq}{equation}
	\Tr_{\mathcal{A}_{N-k}}[X]=\det[X] \Tr_{\mathcal{A}_k}[X^{-1}]\,.
\end{empheq}
Now, since $I(g,g)$ is similar to its inverse, and $\det I(g,g)=1$, this gives
\begin{empheq}{equation}\label{GF:palin}
	\Tr_{\mathcal{A}_{N-k}}[I(g,g)]= \Tr_{\mathcal{A}_k}[I(g,g)]\,,
\end{empheq}
which proves the assertion. Equation \eqref{GF:palin} also shows that the generating function $F_A(t;I(g,g))$ is a palindromic polynomial. 

The main object of study in the remainder of this paper is the function
\begin{empheq}{equation}\label{GF:F.def}
	\FF(t) = \frac1N \ln F_A(t;I(g,g))= \frac1N \Tr \ln [1+tI(g,g)]\,,
\end{empheq}
from which the traces $\Tr_{\mathcal{A}_k}[I(g,g)]$ can be calculated by
\begin{empheq}{equation}\label{GF:F.traces}
	\Tr_{\mathcal{A}_k}[I(g,g)] = \oint \frac{dt}{2\pi i t} \e{N[\FF(t)-\kappa\ln t]}\,,
\end{empheq}
where we have introduced the ratio
\begin{empheq}{equation}\label{GF:kappa.def}
	\kappa= \frac{k}N~.
\end{empheq}
We are interested in the large $N$ regime, keeping the 't~Hooft coupling $\lambda$ and the ratio $\kappa$ fixed. In this regime, the integral in \eqref{GF:F.traces} is dominated by the saddle point value,\footnote{To obtain \eqref{GF:saddle}, introduce $t = t_\ast \e{iz}$, expand the integrand in $z$ up to second order and evaluate the Gaussian integral. The second term in the exponent comes from the Gaussian integral.} 
%
\begin{empheq}{equation}
\label{GF:saddle}
	\Tr_{\mathcal{A}_k}[I(g,g)] = \e{N[\mathcal{F}(t_\ast)-\kappa \ln t_\ast ] 
		- \frac12 \ln [ 2\pi N(\kappa + t_\ast^2 \FF''(t_\ast)) ]}~,
\end{empheq}
where $t_\ast$ satisfies the saddle point equation
\begin{empheq}{equation}\label{GF:t.star}
	t_\ast \FF'(t_\ast) = \kappa~. 
\end{empheq} 
Moreover, $\FF(t)$ admits an asymptotic expansion in $1/N$,
\begin{empheq}{equation}\label{GF:F.N.expand}
	\FF(t) = \sum_{n=0}^\infty \FF[n] N^{-n}~.
\end{empheq}
Our aim is to calculate the terms $\FF[0](t)$ and $\FF[1](t)$ from the exact, but formal, expression \eqref{GF:F.def}.




==> SWL.tex <==

\section{Totally Symmetric Wilson loops}\label{Sec:SWL}
The generating function of traces in the totally symmetric representations of $U(N)$ is
\begin{empheq}{alignat=7}
	F_S\left(t;X\right)&\equiv\frac{1}{\textrm{det}\left[1-tX\right]}&&=\sum_{k=0}^N\textrm{Tr}_{\mathcal{S}_k}\hspace{-0.1cm}\left[X\right]t^k\,.
\end{empheq}
Of course, $F_S(t;X)=1/F_A(-t,X)$. Using the geometric series to represent this as
\begin{empheq}{alignat=7}
	F_S\left(t;X\right)&=\det\left[\sum_{n=0}^{\infty}t^nX^n\right]\,,
\end{empheq}
we can compute the matrix model integrals to find
\begin{empheq}{alignat=7}
	\langle F_S\left(t;e^M\right)\rangle&=\det\left[\sum_{n=0}^{\infty}t^ne^{\frac{n^2g^2}{2}}I(ng,ng)\right]\,.
\end{empheq}
As we have established, at leading order in $1/N$ we can replace
\begin{empheq}{alignat=7}
	I(ng,ng)&=e^{-\frac{n(n-1)g^2}{2}}I(g,g)^n\,.
\end{empheq}
Thus,
\begin{empheq}{alignat=7}
	\langle F_S\left(t;e^M\right)\rangle&=\det\left[\sum_{n=0}^{\infty}t^ne^{\frac{ng^2}{2}}I(g,g)^n\right]
	\\
	&=\frac{1}{\det\left[1-te^{\frac{g^2}{2}}I(g,g)\right]}
	\\
	&=F_S\left(t;e^{\frac{g^2}{2}}I(g,g)\right)\,,
\end{empheq}
and we get the formal result
\begin{empheq}{alignat=7}
	\left\langle W_{\mathcal{S}_k}\right\rangle_{U(N)}&=\frac{1}{\textrm{dim}[\mathcal{S}_k]}e^{\frac{\lambda k}{8N}}\textrm{Tr}_{\mathcal{S}_k}\hspace{-0.1cm}\left[I(g,g)\right]\,.
\end{empheq}

The calculation can be easily extended to an arbitrary generating function of the form
\begin{empheq}{alignat=7}
	F_f\left(t;X\right)&=\det\left[\sum_{n=0}^{\infty}f_nt^nX^n\right]\,,
\end{empheq}
with
\begin{empheq}{alignat=7}
	\langle F_f\left(t;e^M\right)\rangle&=\det\left[\sum_{n=0}^{\infty}f_nt^ne^{\frac{n^2g^2}{2}}I(ng,ng)\right]\,.
\end{empheq}
Again, in the $N\rightarrow\infty$ limit we get
\begin{empheq}{alignat=7}
	\langle F_f\left(t;e^M\right)\rangle&=F_f\left(t;e^{\frac{g^2}{2}}I(g,g)\right)\,.
\end{empheq}

